Multi-GPU Graph Analytics

We present a single-node, multi-GPU programmable graph processing library that allows programmers to easily extend single-GPU graph algorithms to achieve scalable performance on large graphs with billions of edges. Directly using the single-GPU implementations, our design only requires programmers to specify a few algorithm-dependent concerns, hiding most multi-GPU related implementation details. We analyze the theoretical and practical limits to scalability in the context of varying graph primitives and datasets. We describe several optimizations, such as direction optimizing traversal, and a just-enough memory allocation scheme, for better performance and smaller memory consumption. Compared to previous work, we achieve best-of-class performance across operations and datasets, including excellent strong and weak scalability on most primitives as we increase the number of GPUs in the system.

==> table/road.tex <==
\begin{table}
  \centering
  \begin{tabular}{l c r r r}
    \toprule
      group & name & \multicolumn{1}{c}{$|V|$}
                   & \multicolumn{1}{c}{$|E|$}
                   & \multicolumn{1}{c}{$D$}\\
    \midrule
    road & germany\_osm  & 11.5M & 24.7M & 4844$^*$ \\
    road & asia\_osm     & 12.0M & 25.4M & 38576$^*$ \\
    road & road\_central & 14.1M & 33.9M & 4183$^*$ \\
    road & road\_usa     & 23.9M & 57.7M & 6391$^*$ \\
    road & europe\_osm   & 50.9M & 108M  & 19259$^*$ \\
    \bottomrule
  \end{tabular}
  \caption{Road network datasets. $|V|$ and $|E|$ are
    vertex and edge counts; $d$ is the graph diameter, approximated
    using multiple run of random sourced BFS\@.\label{tab:road}}
\end{table}


==> tex/abstraction.tex <==
We present the implementation details of the mGPU layer in this section,
including graph partitioning, the iteration loop, a multi-threads/streams
optimization, and a just-enough automatic memory reallocation scheme.

\subsection{Partitioning of Input Graphs}
At the beginning of the block design, a user-selected graph partitioner assigns
the vertices to different GPUs, and records the assignments in a global
partition table. Based on this table, a GPU hosting a vertex will also host its
neighbor list. Remote vertices in local neighbor lists will have a copy
locally. Vertices may be relabeled in a subgraph to make the vertex IDs
continuous in the subgraph; they can also keep the original vertex IDs, which
is useful for algorithms that need to access vertices more than 1 hop away. The
subgraph forming process will also generate several partition related tables,
such as local partition tables that indicate which GPUs host the vertices in the
subgraph, and conversion tables for converting local and remote IDs
of the same original vertex.

\begin{figure}
  \centering
  \includegraphics[width=0.45\textwidth]{fig/graph_partition-crop.pdf}
  \centering
  \caption{An original undirected graph and its two subgraphs on two GPUs.\label{fig:graph}}

\end{figure}

Figure~\ref{fig:graph} shows a result of the partitioning, with the original
graph on top and two sub-graphs at the bottom. Local vertices are darkened, and
the smaller number next to a vertex is its ID in the other sub-graph. A sample
execution of the mGPU BFS illustrates how an algorithm runs using the
sub-graphs. Suppose the source vertex is $v_1$ in the original graph  The
initial step converts it to $v_0$ on GPU0, and marks the label for $v_0$ on
GPU0 as 0. In iteration 1, GPU0 processes local vertex $v_0$, and marks
labels of $v_3$, $v_4$, and $v_5$ as 1; since these vertices are all hosted on
GPU1, they are converted to $v_0$, $v_1$ and $v_2$, and transmitted to GPU1,
together with their labels. In iteration 2, GPU1 processes local vertices
$v_0$, $v_1$, and $v_2$, and marks the labels for $v_4$, $v_5$, $v_6$ and $v_3$
as 2; $v_4$, $v_5$ and $v_6$ then get converted to $v_0$, $v_1$, $v_2$, and
transmitted to GPU0 with labels 2. However, since the label for $v_0$ on GPU0
is 0, it will not be updated to 2, and $v_0$ will not appear in the input
frontier for the next iteration. Iterations continue until all frontiers are
empty.

\subsection{The Iteration Loop}
\label{subsec:loop}
The key component of the block design is an iteration loop. Gunrock uses a bulk
synchronous parallel model, and processes graph algorithms in iterations. For
most algorithms, the mGPU iteration loop follows the algorithm's iteration, and
computation kernels are placed in sub-queue or full-queue kernel blocks. At the beginning of each iteration, local and remote input
frontiers will go through the sub-queue kernels in parallel.
The output sub-frontiers are then merged, and go through
the full-queue kernels.

At this point, the algorithm will check the convergence condition to decide whether
the iteration loop should stop. Users can specify their own stop conditions.
The stop condition is slightly more complex compared to the single GPU case. On
a single GPU, an empty frontier means there is no more work to do, and the loop
should stop. But for mGPU, peer GPUs may push new frontier elements to a GPU
that has empty frontiers. The stop condition hence needs to guarantee there is
no current or future workload on any GPU or in transmission. Generally, an
algorithm stops if an error is reported by any GPU\@; and it continues if 1)~any
GPU has ongoing work or an non-empty input queue, 2)~any GPU has outgoing data
package to its peers, or 3)~any GPU has received but not yet processed a data
package.

If the loop continues, it will separate the local and remote vertices in the
output frontier according to the local partition tables. The default separation
process first marks a table to indicate whether each vertex in the output
frontier is hosted on individual GPUs, then performs a multiple prefix sum on that
table to get the positions of vertices in their corresponding remote output or
local input frontiers, and finally writes the vertices to those frontiers.
Local input frontiers will be used for the next iteration, and the remote ones
will go through the data packaging process for vertex ID conversion and
user-specified value attachment before being pushed to peer GPUs. Users can
create their own separate blocks as well, such as PageRank's block to put all vertices
in the remote output frontiers by default.

At the other end, the peer GPU will check whether data packages have been
received, and unpack them if they have. The unpackaging step is algorithm-specific: for BFS-like algorithms, it will update the local copy of vertex
associated values, and output the frontier received from the peer GPU to the
sub-queue kernel; for some other algorithms, like connected component, it will
only update the vertex associated values, and output an empty frontier.

As mentioned before, the main computation steps can be placed at the sub-queue
or the full-queue kernel blocks. It is always safe to use the
full-queue option,
since that will force the framework to wait for updates from all peers before
proceeding with the computation. However, if the computation on local input
frontiers does not depend on updated values from peers, then it can be placed
in the sub-queue kernels block to expose more concurrency. For
instance, the BFS algorithm can proceed on the local frontier without updates
from peer GPUs. A vertex will only need to go through the computation again if
a smaller label value for it is received after the computation for the current
iteration is finished. This guarantees the smaller values are the only
effective ones after the merge step at the price of slightly more workload.

\subsection{Multiple Threads, Multiple Streams and Synchronization}
Gunrock uses dedicated CPU threads to control each GPU\@. Within the iteration
loop, CPU threads monitor the status of all GPU operations, including API calls
and kernel launches. Once an error occurs on any GPU, all CPU threads will
break from their loop and the whole program exits. This mechanism effectively
prevents locking caused by GPUs waiting on peers that encounter errors. The CPU
threads also monitor the lengths of all frontiers, to provide them as
parameters for GPU operations, and to judge whether the loop has finished.

Gunrock utilizes GPU streams to overlap computation and data movement. In
Fig.~\ref{fig:block}, each column above the merge block is assigned to
a dedicated GPU stream. All GPU operators in these columns are asynchronous,
and there is no synchronization point in these blocks. This makes the GPU
execution of each column independent, and enables the overlap of local input
frontier computation, received data processing, and outgoing data movement.
This also removes possible false dependencies imposed by the order in which GPU
operations are submitted.  If only a single stream is used, all GPU operations
will execute in the order they are submitted. For example, if the sub-queue
computation kernels are submitted before the received data unpackaging step,
the received data can only be processed after the local frontier computation.
However, these two operations do not depend on each other, and the execution
order of them should not be enforced.

The synchronization point for all streams on a GPU is at the merge step,
because outputs from all sub-frontiers should all be ready at that point for
further processing. Because there is no explicit global
synchronization on GPUs, we ensure the
cooperation of GPUs by setting an event in the stream that
processes the received data, that waits before the unpackaging step until data
from the peer GPU has been received. This preserves the data dependency. More
importantly, a package containing the results from the previous iteration at
a peer GPU indicates the computation of a previous iteration on the peer GPU has
finished. Since the local GPU will not send out packages for the current iteration
before the iteration finishes, the peer GPUs cannot go any further than the
merge step at the next iteration. By doing this, no GPU can go more than one
iteration ahead of its peers, which is necessary for correctness. This loosely
implicit synchronization also increases performance in practice, because data is only
required when it is first used.

\subsection{Just-enough Memory Allocation}
Memory usage is another key aspect of mGPU programming. Minimizing the memory footprint
is essential for mGPU to handle large graphs using limited GPU memory.
However, graphs are irregular data structures, thus it is difficult to know
the maximum size of the frontiers as well as other memory spaces before
actually running an algorithm on a graph.  As
a result, preallocation of worst-case storage requirements is a common
solution.

In order to minimize memory usage while maintaining correctness, we implement
a just-enough memory allocation scheme. The idea is simple: we check the
allocated and the required memory size before all operations that may exceed
the size limit, and reallocate it using the required memory size if the current
size is not enough. If required, the content in the original memory space will
be copied to the new one. We call it just-enough allocation, because if the
initialization step only preallocates a very small amount of memory, a graph
algorithm can still run, and will resize the involved arrays to the actual
required size during the execution. The resulting sizes are the minimal amount
of memory the algorithm needs to run without reallocation, for the given input.

But sometimes the required size is unknown when GPU operations take an array as
output destination. We then have two choices. We can use a lightweight computation just before the
actual operation to compute the size, or use reasonable constraints to figure
out the maximum possible size. For example,
we can compute the prefix sums of neighbor list lengths for vertices in the input
frontier, an operation originally inside the advance step, to
know the resulted frontier size, do a size check, and then continue
with the rest of the advance step.
For arrays that are used for inter-GPU communication, the size
is bounded by the number of vertices adjacent to the cross GPU edges, because
mGPU Gunrock currently only communicates vertex frontiers, and no duplication
can appear in the output frontiers.

Memory reallocation on GPU is expensive, because it needs to wait for all
current tasks on the GPU to finish before performing the
allocation/deallocation in a blocking manner, and only then re-enable the GPU
for other operations. Knowing roughly how much memory is needed and providing
this information to the library can reduce the number of reallocations.
We notice that for a given algorithm, the memory requirement patterns are
similar for graphs of the same kind. For instance, the required frontier sizes
are $\sim8.2$ times of the vertex count for BFS on road networks using 6 GPUs.
The just-enough memory reallocation can make use of this information and do
a preallocation at the initialization step. During the execution, if the
preallocated size is not enough, auto-reallocation takes place, to guarantee
the size of allocated memory is always enough.

In cases when the required memory sizes are known beforehand, the memory
will be preallocated accordingly, and the size checking feature will be turned
off, guaranteeing no reallocation will occur. Disabling size checking
also enables some optimizations for better performance, such as removing the
synchronization used to get the required frontier size on the CPU\@.


==> tex/discussion.tex <==
\input {table/road.tex}
\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{fig/Road.pdf}
  \centering
  \caption{Slowdown of road networks with more GPUs.\label{fig:road}
  \YC{TODO: remove blank spaces}}
\end{figure}

\noindent\textbf{Selection of datasets}
\label{sec:road}
Prior mGPU graph analytics have largely focused on large
scale-free-ish graphs with small diameters. These graphs are easier to
parallelize and scale than high-diameter, low-degree graphs like road
networks (Table~\ref{tab:road}). In fact, scalability is a significant
problem with these graphs on our system (Figure~\ref{fig:road}), and
we expect that if other frameworks evaluated these graphs, they would
see similar results. With our approach, these graphs have insufficient
parallelism to saturate even a single GPU, much less multiple GPUs. As
well, iteration overhead occupies a significant portion of the elapsed
time. As an example, on germany\_osm, the iteration overhead alone is
\{71.4\%, 55\%\} of the total runtime on \{1, 2\} GPUs. Efficiently
running these graphs would require a different approach, perhaps
necessitating preprocessing~\cite{Delling:2010:PHS}.

\noindent\textbf{Partitioner}
Our ideal partitioner has the following properties: 1)~the ability to
use the size of the partition border rather than the number of cutting
edges as its target; 2)~never/rarely downgrades performance
(Fig.~\ref{fig:partitioner}); 3)~preferably computing partitions on
the scale of our processing time (milliseconds) rather than the
seconds of most offline partitioners. It would also run on a single
node (out-of-core) rather than on a cluster. We see this as an
interesting open problem, particularly given that a simple random
partitioner gives the same quality of results in our tests as
biased-random or METIS\@.

\noindent\textbf{Future hardware and scalability}
Upcoming GPUs offer promising improvements that we hope will support
continued performance growth. We ran a handful of experiments on the
consumer-grade Titan~X GPU and achieved a near-doubling of
performance. The newly announced P100 ``Pascal'' GPU has significantly
faster interconnect, memory bandwidth, and memory capacity, and should
be an excellent platform for future work. We note that as future GPUs
improve the hardware-specific terms in the BSP model ($W$ and $g$),
the software-specific terms become even more important.

With our current system, the primitives that scale the best have the
following characteristics: heavy local computation (large $W$), small
communication volume (small $H$, certainly smaller than $W$), and
small iteration count ($S$) (or an iteration count that does not
impact scalability). For example, PR (the easiest primitive to
implement at scale) meets all these three requirements; DOBFS, on the
other hand, has the same order for $W$ and $H$, and its scaling curve
is flat.


==> tex/evaluation.tex <==
\input{table/datasets}
\input{table/compare}

We evaluate five graph primitives on our system: BFS, single-source
shortest path (SSSP),
single-source BC, connected components (CC), and PageRank. This set of
primitives covers the most common basic
graph analytic types mentioned in Section~\ref{sec:intro}. The main purpose of
the evaluation is to explore the performance and scalability of our graph
analytics system, and analyze the factors affecting scalability.

Because primitives for BFS, SSSP and BC share a similar structure (all three are traversal-based primitives), and PageRank and CC are non-traversal-based graph primitives
with a frontier of all vertices at the start, we use BFS to represent the
former and CC to represent the latter in some analyses.

\subsection{Testing Environment and Datasets} We run most tests on nodes with
6 NVIDIA Tesla K40 cards, a 10-core Intel Xeon E5-2690 v2, and 128 GB CPU
memory, running on CentOS 6.4 with CUDA 7.0 (both driver and runtime) and gcc
4.7.3. We complete a small portion of the tests with 4 NVIDIA Tesla
K80 cards (which feature two GPUs on one board, so 8 GPUs in total).
We indicate which tests are performed on the latter. All programs are compiled
with -O3 flag and set to target the actual streaming multiprocessor generation
of the GPU hardware.

The dataset information is listed in Table~\ref{tab:dataset-info} in
six groups. Each contains graphs of a specific topology with various sizes.
The real-world graphs are from the UF sparse matrix
collection~\cite{Davis:1994:UOF} and the Network Data Repository~\cite{Rossi:2015:NDR}.
The ``soc'',``web'' and ``road'' groups are online social networks, web crawls
of different domains, and road
networks respectively. For SSSP, edge values are randomly generated from
[0,64]. We also include two types of synthesized graphs:
R-MAT~\cite{Chakrabarti:2004:R} and random geometric graphs
(RGG)~\cite{Penrose:2003:RGG}. We implement a R-MAT graph generator on top of
the R-MAT generator in the GTgraph library~\cite{Bader:2006:GAS}, replacing the
sprng random number generator with the drand48\_r function. The R-MAT
parameters are A = 0.57, B = 0.19, C = 0.19 and D = 0.05. Edge factors for the rmat\_48
group is 48, the same as the Kronecker graphs commonly used. Edge factors for
the rmat\_2B group are selected to generate just under 2 billion
edges (before self-loop and multiple edge removal). For RGG graphs, the vertices are randomly distributed points in the unit
square. A pair of vertices are considered connected if the Euclidean distance is less than
$0.55 \sqrt{\log n / n}$, where $n$ is the number of vertices in the
graph. This threshold is chosen in order to ensure that the graph is almost
connected~\cite{Davis:1994:UOF}. Graphs in the ``soc'', ``web'' and rmat groups
follow the power-law distribution. Road networks and RGG graphs are more
mesh-like with high diameters; here we call them high-diameter graphs.

All graphs we use in testing are converted to undirected graphs. Self-loops
and duplicates of the same edge are removed from the graphs.
Tests exceeding the single GPU memory limit are excluded from comparisons that
use single-GPU results as the baseline. Our implementation does support graphs larger than
a single GPU's memory size, such as the $\sim$15~GB rmat\_n24\_63 for
BFS\@. This graph takes 191.9~ms on 6
K40s, achieving 10.2 GTEPS,
but since the single GPU result is not available for those datasets, we don't highlight
those results in our figures.

Results for BFS, SSSP, BC and CC are verified against Boost
1.54~\cite{2013:BCL} on a CPU\@. For PageRank, the CPU reference implementation takes too
long (more than one hour) for large datasets, so we only verify our GPU
implementation with small to medium datasets.
\\
\subsection{Overall Results}
Previous mGPU work is commonly evaluated using R-MAT for scalability, but we
do not think that R-MAT results tell the whole story (Section~\ref{subsec:discussion}). We use the R-MAT results to facilitate comparisons
with previous work, and extend our analysis with more data groups and
algorithms in the following part of this section.

\begin{figure}
    \centering
    \includegraphics[width=0.36\textwidth]{fig/_fig12a-crop.pdf}
    \caption{TEPS (Traversed Edges Per Second) for BFS, with rmat\_n20\_1023
    and rmat\_n23\_48 graphs.\label{fig:gteps}}
\end{figure}

As shown in Fig.~\ref{fig:gteps}, we achieve 10.7~GTEPS when running mGPU Gunrock
on 6 K40 GPUs for BFS, using rmat\_n23\_48. Our performance increases to 22.3~GTEPS
using rmat\_n20\_1023. Our edge traversal rate outperforms all previous work on
GPU BFS within a single node and is comparable to work on GPU clusters using
more GPUs (Table~\ref{tab:compare}). For comparison purposes, we
use the same number of GPUs as previous work for the single-node cases.

\begin{figure}
    \centering
    \includegraphics[width=0.36\textwidth]{fig/_fig12b-crop.pdf}
    \caption{Runtime and memory scalability for PageRank with rmat\_n22\_48 on
    K80s.\label{fig:pr}}

\end{figure}

PageRank in mGPU Gunrock shows linear scalability in both runtime and memory
consumption on tests with 8 K80 GPUs (Fig.~\ref{fig:pr}).
For rmat\_n22\_48, it achieves 5.56x speedup with only 1.69x GPU memory usage as
compared to a single GPU\@.

\begin{figure}
    \centering
    \includegraphics[width=0.36\textwidth]{fig/_fig4a-crop.pdf}
    \includegraphics[width=0.36\textwidth]{fig/_fig5a-crop.pdf}
    \caption{Strong scaling on rmat\_n22\_48 (top), weak scaling on
R-MAT graphs (bottom).\label{fig:scaling}}
\end{figure}

Strong and weak scaling are presented in Fig.~\ref{fig:scaling}.
For strong scaling, we use rmat\_n22\_48; for weak scaling, we use R-MAT graphs
with edge factor 48, and keep 180M edges on each GPU\@. Comparing
Fig.~\ref{fig:gteps} and~\ref{fig:scaling}, we can see rmat\_n22\_48 still does
not have enough work to saturate more than 4 K40s for BFS (49.8\% and 34.4\% strong scaling factor for
4 and 6 K40s), and rmat\_n20\_1023 shows a better strong
scaling factor with 82.0\%. Our BFS achieves a 40.6\% weak scaling factor, while
PageRank shows 81.4\% and 40.8\% for strong and weak scaling factors
respectively.

Why does PageRank have a better strong scaling factor than weak scaling
factor? The cross-GPU communication data package size is proportional to
the number of vertices in the graph, and the algorithm has both all-vertices and
all-edges operations. For strong scaling test cases, the number of vertices
is constant, so the communication overhead and the time taken for all-vertices
computation stays the same, which helps PR scale well when the number of edges on
each GPU decreases. But for weak scaling tests, the number of vertices
increases, which not only increases the edge count and all-edges computation
workload, but also increases the communication overhead and workload for
all-vertices computation.

In the rest of this section, we will analyze the test results from different
perspectives and identify the factors affecting scalability, and discuss
improvements that can be done to further increase performance and
scalability.

%\begin{figure*}[ht]
%    \centering
%    \includegraphics[width=0.24\textwidth]{fig/_fig4a-crop.pdf}
%    \includegraphics[width=0.24\textwidth]{fig/_fig4b-crop.pdf}
%    \includegraphics[width=0.24\textwidth]{fig/_fig5a-crop.pdf}
%    \includegraphics[width=0.24\textwidth]{fig/_fig5b-crop.pdf}
%    \caption{From left to right: strong scaling on R-MAT graphs, strong scaling
%    on RGG graphs, weak scaling on R-MAT graphs, weak scaling on RGG graphs.}
%    \label{fig:scaling}
%\end{figure*}

\subsection{Specific Comparisons}

\input{tex/specific-comparisons}

\subsection{Impacts from Primitives}
Communication latency is an issue with any distributed system. GPUs
are no exception: to achieve speedup, GPUs require a large amount of
data to hide latency. For this reason,
mGPU will generally show a performance gain for very large frontiers with small
overhead in mGPU-specific operations, such as data packaging, exchange, and
unpackaging.

\begin{figure}
    \centering
    \includegraphics[width=0.36\textwidth]{fig/_fig3-crop.pdf}
    \caption{Overall speedup vs.\ a single GPU\@. Data is grouped by algorithms;
error bars show minimum and maximum speedups that result when using different
datasets.\label{fig:overall}}

\end{figure}

Fig.~\ref{fig:overall} shows the average speedup with error bars indicating
the minima and the maxima for the five primitives. Four primitives get 3
to 5 times speedup for the best cases (using the R-MAT graphs), while SSSP gets 2. We also observe that
the speedup is primitive- and dataset-specific, and the average performance
improvement is only a few tens of percent, except for PageRank. This low
average is attributed to results from high-diameter graphs, which we will discuss
in the next subsection. We compare BFS and
PageRank to show the difference in Fig.~\ref{fig:bfspr}.

\begin{figure}
    \centering
    \includegraphics[width=0.36\textwidth]{fig/_fig6a-crop.pdf}
    \includegraphics[width=0.36\textwidth]{fig/_fig6c-crop.pdf}
    \caption{Speedup of BFS (top) and PageRank (bottom) for different graph types,
    with error bars showing minima and maxima that result from datasets of the
    same types.\label{fig:bfspr}}
\end{figure}

PageRank outperforms BFS on both
power-law and high-diameter graphs in terms of performance scalability (Fig.~\ref{fig:bfspr}).
We believe the reasons are 1)~the main body of PageRank-based algorithms
are operations on all vertices or all edges, and this guarantees the working
frontiers are always large, even after distribution onto mGPUs; 2)~the data
communication pattern is simple, because GPUs only need to push an associated value
for each remote vertex to its hosting GPU\@. Given the frontiers are the same
for all iterations in PageRank, the data communication can be achieved by
a simple table lookup and a data movement operation.

On the contrary, BFS-based algorithms work on moving frontiers, and the
frontier sizes are data-dependent. For datasets that can provide large
frontiers most of the time, like rmat\_48 and rmat\_2B, enough workload can be
sent to the GPUs to keep them fully occupied; but for datasets that generate small frontiers, GPUs are
underutilized. The data communication pattern is more complex for this class of
algorithms, as stated in Section~\ref{subsec:loop}---it requires marking,
multiple prefix-sum computation, vertex ID conversion, and associated value packaging---
before sending the remote output frontiers to peer GPUs. For small frontiers, the
overhead of these operations is significant. These two factors together can make
performance suffer on mGPU, as shown by the four primitives on
the RGG dataset.

To overcome these two limits, a primitive needs to have large frontiers in most
iterations, and simple operations for data exchange. The former is data-dependent, and can be achieved by either algorithm design or being able to guarantee there is enough
data to saturate all the GPUs for most iterations. The latter may be
achieved by sending the whole output frontier to all peer GPUs, but the
tradeoff between computation and communication needs to be carefully
studied.

\subsection{Impacts from Datasets}
\begin{figure}
    \centering
    \includegraphics[width=0.36\textwidth]{fig/_fig8a-crop.pdf}
    \includegraphics[width=0.36\textwidth]{fig/_fig8b-crop.pdf}
    \caption{Speedup of R-MAT (top) and RGG (bottom) graphs for five algorithms,
with error bars indicating minima and maxima from different
datasets of the same graph types.\label{fig:rmatrgg}}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{fig/_fig7-crop.pdf}
    \caption{Input frontier sizes at different iterations for R-MAT
graph, social and road networks.\label{fig:frontier}}
\end{figure}

Graph topologies also affect the frontier sizes and mGPU operation overhead.
Fig.~\ref{fig:rmatrgg} shows the speedup of all primitives for R-MAT and RGG
graphs, while Fig.~\ref{fig:frontier} shows the frontier sizes per
BFS iteration. Vertices in R-MAT graphs have high average out-degrees.
This leads to huge frontiers for all GPUs in certain iterations, and those
iterations account for most of the computation time. GPUs in these iterations
are fully utilized. Diameters for R-MAT graphs are small, so the number of
iterations for BFS-based algorithms are limited. This helps in reducing the
total overhead of mGPU operations. Social networks, web graphs and other power-law graphs are similar to R-MAT graphs in these aspects. For web graphs,
the diameters are about twice as high as social networks and R-MAT graphs; the
mGPU operation overhead can be more significant, which may bring speedups down
when more GPUs are used.

On the other hand, RGG graphs, as well as other high-diameter graphs like road
networks, have a low average
edge-to-vertex ratio. This means frontier sizes increase slowly, stay at
around the same level, then come down slowly. The frontier never
reaches a large enough size
to fully utilize even a single GPU, so the utilization for mGPU is even worse. The
high diameter also means high iteration counts for BFS-based algorithms, which
amplifies the effect of mGPU operation overhead. Since frontiers are small, single-GPU
computation is fast, so we see poor scalability on these graphs.

The average speedups are mostly close to the maxima in Fig.~\ref{fig:rmatrgg}, which indicates the effect of dataset sizes. Only one or
two datasets with small sizes in each group get about half of the average
speedup; all other datasets have similar results. This shows that after some
threshold, the speedup only has small variance for the same kind of graphs regardless of
scale.

We considered that GPU-GPU communication bandwidth could be
a bottleneck for good scalability. This is true if entire edge frontiers are transmitted, because their size
can be extremely large (several hundred million for rmat\_n23 and
rmat\_n24). However, if communication is only used on vertex frontiers, as in our
mGPU framework, the transmitted frontier size is small (at most a few millions).
Together with their associated values, the size of all data transmitted
to/from one GPU at any iteration is generally under 100~MB, which only takes a few
ms to pass through the PCIe 3.0 x 16 links. This constitutes a small
portion of total computation time. But within a GPU cluster, the
communication bandwidth is a more significant issue, as multiple GPUs on a node need to
share the inter-node network, which has lower bandwidth and higher latency than PCIe
links. We certainly anticipate that high-bandwidth, low-latency
inter-node communication for GPUs is vital for good scalability on GPU clusters.

Exchange of a very small amount of data between GPU and CPU is a common
occurrence for keeping
track of GPU operation status and the resulted frontier sizes. It often happens
that these frontier sizes are parameters to subsequent GPU operations,
which imposes a synchronization requirement to get those sizes to the CPU\@.
The cross-GPU data packages can also be small, for BFS-like algorithms on
high-diameter graphs, as well as the first and last few iterations of other graphs.
It is not the bandwidth but instead the latency that plays the
important role here. The NVLink CPU-GPU interface~\cite{NVIDIA:2014:NNH} proposed for next generation GPUs, which has much less inter-GPU and CPU-GPU
communication latency, is promising for alleviating these issues.

Graph topologies are not a factor that can be ``solved'' for better
scalability. Nevertheless, techniques like hybrid CPU-GPU computing that only brings the GPU
into action when the frontier size crosses a certain threshold may help~\cite{Gharaibeh:2013:TAG}.

\subsection{Impacts from Memory Allocation Methods}
\begin{figure}
    \centering
    \includegraphics[width=0.36\textwidth]{fig/_fig9a-crop.pdf}
    \includegraphics[width=0.36\textwidth]{fig/_fig9b-crop.pdf}
    \caption{Full preallocation vs.\ just-enough reallocation comparison on
    speed (top, higher is better) and memory usage (bottom, lower is better)
    on different graph types for BFS\@. Error bars indicate the minima and
    maxima resulting from different datasets of the same graph types.\label{fig:justenough}}
\end{figure}

Memory is another important aspect of mGPU scalability. Ideally, the total GPU
memory consumption should be close to that on single GPU, but in practice extra
memory is allocated for duplicated information, the partition table, transmission
data package, etc. It is desirable that this additional memory usage is small, so
that mGPU can deal with larger graphs. Graph problems impose a significant
challenge on memory: the frontier sizes are unknown a priori. We implement
a just-enough memory allocation scheme to deal with this issue. The effect of
the scheme on BFS is shown in Fig.~\ref{fig:justenough}. We run tests under two
conditions: 1)~using minimum preallocation and auto-reallocation, and 2)~using
suitable preallocation size (as reported by the previous iteration) and
turning off size-checking. The upper graph shows the speedup under testing
condition 2 vs.\ 1, and the lower graph shows the respective memory usage
comparison.

We can see that runtime improves significantly if no reallocation is required,
but at the cost of using more memory. It gets about 2x speedup for power-law graphs when reallocation does not occur, but high-diameter graphs gain
almost no benefit in performance. This is because the frontier sizes keep
increasing for the first half of iterations on power-law graphs, which means
reallocation happens for half of the iterations; but for high-diameter graphs,
frontier size are mostly within a range, and reallocation only happens for a
small number of iterations. The speedup is more significant
if more GPUs are used, because a higher GPU count results in more arrays used, leading to
more resizing for condition 1. The high speedups are contributed by the
small datasets in each group, because the total runtime is small and the
reallocation time can be a large fraction of that.

Currently we only profile the
memory usage using two main factors: how much memory is required for frontiers and
communication, both with respect to the number of vertices in the sub-graphs.
Extra preallocation happens when these two factors are different across GPUs, and
we will select the maximum. We cannot and should not compute different memory sizes
for each individual GPU, because there is no guarantee from the
partitioner that the same portion of graph will be assigned to the same GPU
each time. What can be guaranteed is that these factors are similar for graphs
of the same kind and can be used for the same primitives.

The results in other parts of this section are all taken with suitable size
memory preallocated and size checking turned off. To our knowledge, no previous
work has explored similar features like just-enough allocation.

\begin{figure}
    \centering
    \includegraphics[width=0.36\textwidth]{fig/_fig10-crop.pdf}
    \caption{Overall memory scaling for different algorithms, using
just-enough reallocation.\label{fig:memory}}
\end{figure}

Figure~\ref{fig:memory} shows the minimum memory usage as compared to
using a single GPU\@. The average total usage is about 2 times for 6 GPUs. The
large maxima are mostly for RGG graphs and road networks, which have low edge-to-vertex
ratios. mGPU Gunrock duplicates vertices and associated values; these
make up most of the additional memory usage on the aforementioned two graph types. But since the
original single-GPU memory consumption is not high for these graphs ($\sim$2.6GB for
rgg\_25), the high memory usage increase for these particular datasets is not
a problem.

\subsection{Impacts from Partitioner}
\label{subsec:partitioner}
\begin{figure}
    \centering
    \includegraphics[width=0.36\textwidth]{fig/_fig11a-crop.pdf}
    \includegraphics[width=0.36\textwidth]{fig/_fig11b-crop.pdf}
    \caption{Normalized runtime comparison of different partitioners with the
    runtime of the uniform random partitioner set to 1. Top: BFS, bottom: CC\@.
    The partition\_time for Metis is much greater than the random partitioner.
For BFS, it is 33.8 (times compared to the uniform random partitioner) on average and 131.3 at maximum, and for
CC it is 161.3
on average and 597.2 at maximum.\label{fig:partitioner}}

\end{figure}

We try different graph partitioning strategies to analyze their partitioning
time as well as the impacts on algorithm runtime, workload redundancy, and
memory usage. The partitioners are:
\begin{description}[style=unboxed, leftmargin=0cm]
\setlength{\itemsep}{0.1cm}
\setlength{\parskip}{0.1cm}
    \item[rand] Random partitioner: vertices are randomly assigned to GPUs;
    \item[static] Static partitioner: vertex $v$ is assigned to GPUv $\bmod$
\#GPUs;
    \item[metis] the Metis partitioner~\cite{Karypis:1998:FHQ} with default settings;
    \item[brp] Bias random partitioner: the assignment is biased by how many
neighbors have already been assigned to the GPUs, and it tends to put
neighbors together. The partitioning factor adjusts the bias effect, 0 for no
bias at all, and 1 for fully biased.
\end{description}

Figure~\ref{fig:partitioner} shows the results compared to the random
partitioner. Workload in the figure indicates how much work is done in the
test, e.g., in terms of number of edges traversed or items processed.
The mGPU implementation may perform redundant work. Good partitioning results
can keep the redundancy at a minimum. The rand and static partitioners are
similar, and the simple method in static partitioner keeps the partition
time small.

Metis can reduce runtime and memory usage of BFS to about half as compared to
the random partitioner, because the smaller number of cross-GPU edges help to
reduce both data movement and the space required for mGPU\@.  But the shortcomings
are significant: it takes much longer to partition large graphs,
even longer than the actual runtime of the
GPU primitives and the random partitioner; it is not suitable for all algorithms,
and results in longer runtime than the random partitioner for CC despite the
workload being less; and it also produces subgraphs that have very different memory
usage patterns, which makes it difficult to provide the allocation factors that
the just-enough memory allocation needs. In general, Metis can be used for
BFS-based algorithms, but it is not an ideal graph partitioner for mGPU
graph processing in general.

The bias random partitioner reveals more information. For BFS, when the
partition factor is closer to 1, i.e., vertices are more likely to be on the
same GPU with their neighbors, the space required for communication is smaller.
But that doesn't affect the runtime. For CC, being closer to neighbors may not
be a good thing, because we actually observe an increase in runtime.

So far, we have not seen a good graph partitioner that performs well in all
four aspects.

\subsection{Discussion}
\label{subsec:discussion}
From the above evaluations, we offer two general insights on evaluating
multi-GPU graph analytics frameworks.
\begin{description}[style=unboxed, leftmargin=0cm]
\setlength{\itemsep}{0.1cm}
\setlength{\parskip}{0.1cm}
\item[On Graph Primitives] We see very different results regarding performance
    and scalability on two different types of graph algorithms. PageRank, as
    a representative of non-traversal-based graph algorithms with dense
    computation, achieves high performance and approaches linear scalability  on all datasets.
    This is because of its cross-iteration and cross-GPU load balancing and
    predictable memory access and control flow (the PageRank
    computation always visits all neighbors of
    an element). PageRank is a best-case scenario for scalability, and
    thus we submit that a full evaluation of a framework should also
    include graph algorithms with more
    workload irregularity and cross-GPU load imbalance.
\item[On Graph Datasets] Among the many synthesized and real-world
  datasets that we used for evaluation, we note that R-MAT
    graphs always yield the best peak performance and approach linear scalability. Although R-MAT
    was designed to represent the structure of scale free graphs, our results
    suggest that it actually performs quite differently from other
    datasets, including real-world scale-free graphs, on which we
    achieve less ideal scalability, or even fail to
    scale at all. We submit that while R-MAT results can be used to
    show impressive numbers, graph analytics frameworks must demonstrate
    performance on a wide range of datasets for a proper evaluation.
\end{description}


==> tex/specific-comparisons.tex <==
\begin{table*}
\small
\begin{tabular}{lp{1.5in}lp{2.5in}l}
\toprule
Prior Work & Machine & Primitive & Dataset &
Performance\\ % & Gunrock Runtime (MTEPS) \\
\midrule
% Bisson
Bisson~\cite{Bisson:2015:PDB} & 4 nodes, 1$\times$K20X/node & BFS
& com-Orkut undirected (V=3M, E=117M) & 2.67~GTEPS\\
Bisson~\cite{Bisson:2015:PDB} & 64 nodes, 1$\times$K20X/node & BFS
& com-Friendster undirected (V=65.6M, E=1.8B) & 15.68~GTEPS\\
Bisson~\cite{Bisson:2015:PDB} & 4096 nodes, 1$\times$K20X/node & BFS
& kron-logn33\_16 (undirected)& $\sim$400~GTEPS\\
% Bernaschi
Bernaschi~\cite{Bernaschi:2015:EGD} & 4 nodes, 1$\times$K20X/node (Piz-Daint Aries) & BFS
& kron-logn23\_16 (undirected?) & $\sim$1.3~GTEPS\\
Bernaschi~\cite{Bernaschi:2015:EGD} & 16 nodes, 1$\times$K20X/node (Piz-Daint Aries) & BFS
& kron-logn25\_16 (undirected?) & $\sim$3.2~GTEPS\\
Bernaschi~\cite{Bernaschi:2015:EGD} & 64 nodes, 1$\times$K20X/node (Piz-Daint Aries) & BFS
& kron-logn27\_16 (undirected?) & $\sim$10~GTEPS\\
Bernaschi~\cite{Bernaschi:2015:EGD} & 256 nodes, 1$\times$K20X/node (Piz-Daint Aries) & BFS
& kron-logn29\_16 (undirected?) & $\sim$22.5~GTEPS\\
Bernaschi~\cite{Bernaschi:2015:EGD} & 1024 nodes, 1$\times$K20X/node (Piz-Daint Aries) & BFS
& kron-logn31\_16 (undirected?) & $\sim$43~GTEPS\\
% Fu weak scaling
Fu~\cite{Fu:2014:PBF} & 2 nodes, 2$\times$K20/node (SCI) & BFS & kron-logn23\_16 (undirected) & 6.3~GTEPS\\
Fu~\cite{Fu:2014:PBF} & 8 nodes, 2$\times$K20/node (SCI) & BFS & kron-logn25\_16 (undirected) & 15~GTEPS\\
Fu~\cite{Fu:2014:PBF} & 32 nodes, 2$\times$K20/node (SCI) & BFS
& kron-logn25\_16 (undirected)& 22.7~GTEPS\\
Fu~\cite{Fu:2014:PBF} & 32 nodes, 2$\times$K20/node (SCI) & BFS
& kron-logn27\_16 (undirected) & 29.1~GTEPS\\
% Bebee
Bebee~\cite{Bebee:2016:WTD} & 16$\times$K40 & BFS
& ICWSM 2010 Twitter dataset (E=1.9B) & 0.2242~s\\ % runtime data from video

% Liu/Enterprise strong scaling
Liu~\cite{Liu:2015:EBG} & 2$\times$ K40 & BFS
& kron-logn24\_32 (undirected) & 15~GTEPS\\
Liu~\cite{Liu:2015:EBG} & 4$\times$ K40 & BFS
& kron-logn24\_32 (undirected)  & 18~GTEPS\\
Liu~\cite{Liu:2015:EBG} & 8$\times$ K40 & BFS
& kron-logn24\_32 (undirected)  & 18.4~GTEPS\\

%Sengupta, GraphReduce, the SC15 streaming / out of core paper
Sengupta~\cite{Sengupta:2015:GPL} & 1$\times$ K40c & BFS
& kron-logn21\_16 (directed) & 4 sec\\
Sengupta~\cite{Sengupta:2015:GPL} & 1$\times$ K40c & SSSP
& kron-logn21\_16 (directed) & 7 sec\\
Sengupta~\cite{Sengupta:2015:GPL} & 1$\times$ K40c & PR$^{1}$
& kron-logn21\_16 (directed) & 93 sec\\
Sengupta~\cite{Sengupta:2015:GPL} & 1$\times$ K40c & CC
& kron-logn21\_16 (directed) & 9 sec\\
%uk-2002 is the largest dataset they use for out of core, kind of pointless
%when it can fit into a single GPU memory
Sengupta~\cite{Sengupta:2015:GPL} & 1$\times$ K40c & BFS
& uk-2002 (V=18.5M, E=298.1M) & 49 sec\\
Sengupta~\cite{Sengupta:2015:GPL} & 1$\times$ K40c & SSSP
& uk-2002 (V=18.5M, E=298.1M) & 80 sec\\
Sengupta~\cite{Sengupta:2015:GPL} & 1$\times$ K40c & PR$^{1}$
& uk-2002 (V=18.5M, E=298.1M) & 153 sec\\
Sengupta~\cite{Sengupta:2015:GPL} & 1$\times$ K40c & CC
& uk-2002 (V=18.5M, E=298.1M) & 162 sec\\

%Lee, GraphMap, the SC15 cpu cluster paper
Lee~\cite{Lee:2015:SIG} & 21 nodes, 4 cores and 12GB memory per node & SSSP
& uk-2005 (V=39M, E=936M) & 156 sec\\
Lee~\cite{Lee:2015:SIG} & 21 nodes, 4 cores and 12GB memory per node & CC
& uk-2005 (V=39M, E=936M) & 706 sec\\
Lee~\cite{Lee:2015:SIG} & 21 nodes, 4 cores and 12GB memory per node & PR
(per-iteration)
& uk-2005 (V=39M, E=936M) & 57 sec\\

%twitter is the largest dataset they use for a cluster, it can be fit nicely
%inside the GPU memory
Lee~\cite{Lee:2015:SIG} & 21 nodes, 4 cores and 12GB memory per node & SSSP
& twitter (V=42M, E=1.5B) & 150 sec\\
Lee~\cite{Lee:2015:SIG} & 21 nodes, 4 cores and 12GB memory per node & CC
& twitter (V=42M, E=1.5B) & 304 sec\\
Lee~\cite{Lee:2015:SIG} & 21 nodes, 4 cores and 12GB memory per node & PR
(per-iteration)
& twitter (V=42M, E=1.5B) & 149 sec\\

%Frog, the Asynchronous paper
%BFS Results
Shi~\cite{Shi:2015:OAG} & 1$\times$ K20m & BFS & Amazon (V=735K, E=5M) & $^{2}$4.97ms\\
Shi~\cite{Shi:2015:OAG} & 1$\times$ K20m & BFS & DBLP (V=986K, E=7M) & $^{2}$3.38ms\\
Shi~\cite{Shi:2015:OAG} & 1$\times$ K20m & BFS & WikiTalk (V=2K, E=5M) & $^{2}$3.53ms\\
Shi~\cite{Shi:2015:OAG} & 1$\times$ K20m & BFS & LiveJournal (V=5M, E=68M) & $^{2}$7.48ms\\
Shi~\cite{Shi:2015:FAG} & 1$\times$ K20m & BFS & Youtube (V=1M, E=3M) & $^{2}$5.64ms\\
Shi~\cite{Shi:2015:FAG} & 1$\times$ K20m & BFS & Twitter (V=42M, E=1B) & $^{2}$58.8s\\

%SSSP Results
Shi~\cite{Shi:2015:FAG} & 1$\times$ K20m & SSSP & Amazon (V=735K, E=5M) & $^{2}$15.7ms\\
Shi~\cite{Shi:2015:FAG} & 1$\times$ K20m & SSSP & DBLP (V=986K, E=7M) & $^{2}$12.3ms\\
Shi~\cite{Shi:2015:FAG} & 1$\times$ K20m & SSSP & WikiTalk (V=2K, E=5M) & $^{2}$12.0ms\\
Shi~\cite{Shi:2015:FAG} & 1$\times$ K20m & SSSP & Youtube (V=1M, E=3M) & $^{2}$11.2ms\\
Shi~\cite{Shi:2015:FAG} & 1$\times$ K20m & SSSP & Twitter (V=42M, E=1B) & $^{2}$153s\\

%CC Results
Shi~\cite{Shi:2015:FAG} & 1$\times$ K20m & CC & Amazon (V=735K, E=5M) & $^{2}$8.72ms\\
Shi~\cite{Shi:2015:FAG} & 1$\times$ K20m & CC & DBLP (V=986K, E=7M) & $^{2}$9.21ms\\
Shi~\cite{Shi:2015:FAG} & 1$\times$ K20m & CC & WikiTalk (V=2K, E=5M) & $^{2}$11.1ms\\
Shi~\cite{Shi:2015:FAG} & 1$\times$ K20m & CC & Youtube (V=1M, E=3M) & $^{2}$6.18ms\\
Shi~\cite{Shi:2015:FAG} & 1$\times$ K20m & CC & Twitter (V=42M, E=1B) & $^{2}$35s\\

%PR Results
Shi~\cite{Shi:2015:OAG} & 1$\times$ K20m & PR$^{3}$ & Amazon (V=735K, E=5M) & $^{2}$34.7ms\\
Shi~\cite{Shi:2015:OAG} & 1$\times$ K20m & PR$^{3}$ & DBLP (V=986K, E=7M) & $^{2}$50.8ms\\
Shi~\cite{Shi:2015:OAG} & 1$\times$ K20m & PR$^{3}$ & WikiTalk (V=2K, E=5M) & $^{2}$75.1ms\\
Shi~\cite{Shi:2015:FAG} & 1$\times$ K20m & PR$^{3}$ & Youtube (V=1M, E=3M) & $^{2}$35.7ms\\
Shi~\cite{Shi:2015:FAG} & 1$\times$ K20m & PR$^{3}$ & Twitter (V=42M, E=1B) & $^{2}$145s\\
\bottomrule
\label{tab:all-compare}
\end{tabular}
\caption{Summary of prior work in graph analytics.\\ Note 1: damping factor 0.15, no convergence criteria given. \Carl{Damping criteria 0.15 according to their paper, but this could be a typo since most damping factors are 0.85}\\ Note 2: indicates non-trivial amount of preprocessing for asynchronous processing not accounted for in runtime.\\ Note 3: damping factor 0.85, precision 0.005f.}
\end{table*}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main.tex"
%%% End:

